ChartMoE: Mixture of Diversely Aligned Expert Connector for Chart Understanding

Automatic chart understanding is crucial for content comprehension and document parsing. Multimodal Large Language Models (MLLMs) have demonstrated remarkable capabilities in chart understanding through domain-specific alignment and fine-tuning. However, current MLLMs still struggle to provide faithful data and reliable analysis only based on charts. To address it, we propose ChartMoE, which employs the Mixture of Expert (MoE) architecture to replace the traditional linear projector to bridge the modality gap. Specifically, we train several linear connectors through distinct alignment tasks, which are utilized as the foundational initialization parameters for different experts. Additionally, we introduce ChartMoE-Align, a dataset with nearly 1 million chart-table-JSON-code quadruples to conduct three alignment tasks (chart-table/JSON/code). Combined with the vanilla connector, we initialize different experts diversely and adopt high-quality knowledge learning to further refine the MoE connector and LLM parameters. Extensive experiments demonstrate the effectiveness of the MoE connector and our initialization strategy, e.g., ChartMoE improves the accuracy of the previous state-of-the-art from 80.48\% to 84.64\% on the ChartQA benchmark.

==> Fig/texs/chat_example.tex <==
\begin{figure}[h]
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{Fig/figs/chat/chat_edit.png}
        \captionsetup{skip=5pt}
        \caption{xxx}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{Fig/figs/chat/chat_highlight.png}
        \captionsetup{skip=5pt}
        \caption{xxx}
    \end{subfigure}%
    \centering
    \captionsetup{skip=3pt}
    \caption{xxx}
    \label{fig_chat_example}
\end{figure}



==> Tab/tab_chartfc.tex <==
\begin{table}[t]
\centering
\captionsetup{skip=0pt}
\caption{The zero-shot accuracy (\%) performance on \textbf{\textit{ChartFC}} and \textbf{\textit{ChartCheck}}. $\dagger$: supervised training with instructions provided by ChartGemma.}
\resizebox{0.5\linewidth}{!}{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}c|c|cc@{}}
\toprule[1.5pt]
\multirow{2}{*}{Models} & \multirow{2}{*}{ChartFC} & \multicolumn{2}{c}{ChartCheck} \\ \cmidrule(l){3-4} 
 &  & T1 & T2 \\ \midrule
PaliGemma~\cite{paligemma} & 58.26 & 67.34 & 68.50 \\
LLaVA-v1.5$\dagger$~\cite{llava} & 61.28 & 70.22 & 70.03 \\
InternlmXC-v2~\cite{internlm-xcomposerv2} & 65.93 & 72.04 & 70.44 \\
ChartInstruct-LLama2~\cite{chartinstruct} & 69.57 & 70.11 & 68.80 \\
ChartInstruct-FlanT5XL~\cite{chartinstruct} & 70.27 & 72.03 & 73.80 \\
ChartGemma~\cite{chartgemma} & 70.33 & 71.50 & 74.31 \\
\rowcolor{blue!5} ChartMoE (Ours) & 74.73 & 78.87 & 79.20 \\ \bottomrule[1.5pt]
\end{tabular}
}
\vspace{-15pt}
\label{tab_chartfc}
\end{table}



==> Tab/tab_chartmimic.tex <==
\begin{table}[h]
\centering
\captionsetup{skip=3pt}
\caption{The ChartMimic leaderboard with \textbf{\textit{Direct}} Mimic task.}
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{10pt}
\begin{tabular}{@{}c|c|c|cccc|c@{}}
\toprule[1.5pt]
Model & Params & Exec. Rate & Text & Layout & Type & Color & Avg. \\ \midrule
GPT-4O & - & 91.60 & 80.70 & 88.90 & 76.90 & 68.10 & 78.70 \\
GPT-4V & - & 91.40 & 74.30 & 87.10 & 73.80 & 62.10 & 74.30 \\
Claude-3-opus & - & 86.40 & 61.80 & 79.00 & 45.30 & 37.90 & 56.00 \\
InternVL2-Llama3-76B & 76B & 80.40 & 51.10 & 70.20 & 49.40 & 42.70 & 53.40 \\
GeminiProVision & - & 64.20 & 36.90 & 58.60 & 45.10 & 39.60 & 45.00 \\
InternVL2-26B & 26B & 66.40 & 36.10 & 55.40 & 35.40 & 32.80 & 39.90 \\
Phi-3-Vision & 4.2B & 66.00 & 36.40 & 45.00 & 39.00 & 34.30 & 38.70 \\
InternVL2-4B & 4B & 67.60 & 33.30 & 53.30 & 28.60 & 28.30 & 35.90 \\
MiniCPM-Llama3-V2.5 & 8.4B & 58.20 & 22.50 & 40.10 & 31.40 & 26.60 & 30.20 \\
InternVL-Chat-V1.5 & 26B & 60.00 & 26.90 & 42.10 & 26.10 & 24.90 & 30.00 \\
\rowcolor{blue!5}ChartMoE (Ours) & 8B & 53.59 & 18.48 & 50.17 & 31.54 & 19.14 & 29.83 \\
\rowcolor{blue!5}InternlmXC-v2 & 8B & 46.00 & 13.65 & 38.53 & 30.44 & 24.82 & 24.82 \\
Cogvlm2-llama3-chat-19B & 19.2B & 51.40 & 20.60 & 31.10 & 21.70 & 20.00 & 23.30 \\
LLaVA-Next-Mistral-7B & 7.6B & 57.60 & 11.30 & 31.50 & 22.30 & 21.90 & 21.80 \\
DeepSeek-VL-7B & 7.3B & 39.00 & 13.80 & 26.40 & 23.90 & 19.00 & 20.80 \\
LLaVA-Next-Yi-34B & 34.8B & 45.60 & 11.40 & 26.70 & 18.20 & 16.60 & 18.20 \\
IDEFICS2-8B & 7.6B & 42.40 & 5.70 & 28.40 & 11.90 & 10.90 & 14.20 \\
LLaVA-Next-Vicuna-13B & 13.4B & 11.60 & 1.90 & 5.70 & 4.00 & 4.30 & 4.00 \\
LLaVA-Next-Vicuna-7B & 7.1B & 6.20 & 0.80 & 2.10 & 1.40 & 1.60 & 1.60 \\
Qwen-VL-Chat & 9.6B & 4.00 & 0.50 & 2.80 & 1.10 & 0.80 & 1.30 \\ 
\bottomrule[1.5pt]
\end{tabular}
}
\label{tab_chartmimic_direct}
\end{table}

\begin{table}[h]
\centering
\captionsetup{skip=3pt}
\caption{The ChartMimic leaderboard with \textbf{\textit{Customized}} Mimic task.}
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{10pt}
\begin{tabular}{@{}c|c|c|cccc|c@{}}
\toprule[1.5pt]
Model & Params & Exec. Rate & Text & Layout & Type & Color & Avg. \\ \midrule
GPT-4o & - & 94.00 & 79.40 & 91.80 & 81.20 & 68.40 & 80.20 \\
GPT-4V & - & 93.20 & 77.40 & 89.20 & 78.30 & 65.60 & 77.60 \\
InternVL2-Llama3-76B & 76B & 85.60 & 55.90 & 76.80 & 62.60 & 51.00 & 61.60 \\
Claude-3-opus & - & 88.20 & 65.20 & 82.80 & 48.20 & 39.60 & 58.90 \\
GeminiProVision & - & 74.00 & 47.20 & 64.90 & 56.00 & 46.40 & 53.60 \\
InternVL2-26B & 26B & 72.20 & 44.20 & 61.10 & 44.60 & 36.80 & 46.70 \\
\rowcolor{blue!5}ChartMoE (Ours) & 8B & 70.60 & 42.26 & 62.97 & 45.48 & 33.23 & 45.98 \\
\rowcolor{blue!5}InternlmXC-v2 & 8B & 63.40 & 37.09 & 59.87 & 47.87 & 33.22 & 44.51 \\
MiniCPM-Llama3-V2.5 & 8.4B & 69.20 & 40.00 & 53.90 & 43.10 & 35.80 & 43.20 \\
Phi-3-Vision & 4.2B & 67.20 & 30.90 & 52.50 & 46.60 & 42.00 & 43.00 \\
InternVL2-4B & 4B & 70.00 & 37.80 & 51.60 & 40.90 & 35.50 & 41.40 \\
DeepSeek-VL-7B & 7.3B & 55.20 & 28.20 & 45.80 & 40.40 & 33.50 & 37.00 \\
LLAVA-Next-Vi-34B & 34.8B & 59.40 & 33.40 & 45.10 & 26.20 & 24.90 & 32.40 \\
InternVL-Chat-V1.5 & 26B & 48.60 & 30.10 & 38.20 & 27.40 & 22.50 & 29.50 \\
IDEFICS2-8B & 7.6B & 52.40 & 23.60 & 33.50 & 24.10 & 16.20 & 24.40 \\
LLAVA-Next-Mistral-7B & 7.6B & 48.00 & 21.80 & 30.40 & 22.00 & 21.70 & 24.00 \\
Cogvlm2-llama3-chat-19B & 19.2B & 37.80 & 19.10 & 25.60 & 17.60 & 17.10 & 19.90 \\
LLAVA-Next-Vicuna-13B & 13.4B & 32.20 & 9.30 & 21.50 & 17.40 & 14.20 & 15.60 \\
LLAVA-Next-Vicuna-7B & 7.1B & 8.40 & 4.80 & 4.80 & 3.60 & 3.00 & 3.40 \\
Qwen-VL-Chat & 9.6B & 6.80 & 2.60 & 3.80 & 3.50 & 2.60 & 3.20 \\ 
\bottomrule[1.5pt]
\end{tabular}
}
\label{tab_chartmimic_customized}
\end{table}




==> Tab/tab_data_ablation.tex <==
\begin{table}[t]
\centering
\captionsetup{skip=0pt}
\caption{Ablation study on the training strategy, about the alignment stage, high-quality knowledge learning period and chart-specific anneal tuning period.}
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{8pt}
\begin{tabular}{@{}cccc@{}}
\toprule[1.5pt]
\multicolumn{1}{c|}{\multirow{2}{*}{\name\ Recipe}} & \multicolumn{3}{c}{Relax Acc @0.05}  \\ \cmidrule(l){2-4} 
\multicolumn{1}{c|}{} & Human & Aug. & \multicolumn{1}{c}{Avg.} \\ \midrule
\multicolumn{1}{l|}{Baseline: InternlmXC-v2 + ChartQA} & 63.68 & 87.68 & \multicolumn{1}{c}{75.68} \\ \midrule
\multicolumn{1}{l|}{+ \textit{table-JSON-code} Aligned Connector} & 64.24 & 90.16 & \multicolumn{1}{c}{77.20} \\ \midrule
\multicolumn{1}{l|}{+ \textit{Top2-in-4} ChartMoE} & 67.92 & 89.60 & \multicolumn{1}{c}{78.76} \\ \midrule
\multicolumn{1}{l|}{+ \textit{MMC} High-Quality Knowledge Learning} & 67.84 & 90.24 & \multicolumn{1}{c}{79.04} \\ \midrule
\multicolumn{1}{l|}{+ \textit{ChartGemma} Instructions} & \textbf{71.36} & \textbf{91.04} & \multicolumn{1}{c}{\textbf{81.20}}\\ 
\bottomrule[1.5pt]
\end{tabular}
}
\label{tab_data_ablation}
\end{table}


==> Tab/tab_model_ablation.tex <==
\begin{table}[t]
\centering
\captionsetup{skip=0pt}
\caption{Ablation study on three factors in ChartMoE architecture: the number of experts, the number of activated and the initialization of experts. All experiments are conducted on ChartQA training data and evaluated on ChartQA test set.}
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{8pt}
\begin{tabular}{@{}cccccc@{}}
\toprule[1.5pt]
\multicolumn{1}{c|}{\multirow{2}{*}{\makecell{Total\\Experts}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\makecell{Activated\\Experts}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\makecell{Experts\\Initialization}}} & \multicolumn{3}{c}{Relax Acc @0.05} \\ \cmidrule(l){4-6} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & Human & Aug. & Avg. \\ \midrule
\multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{Random} & 59.68 & 86.72 & 73.20 \\ \midrule
\multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{Aligned Co-Upcycle} & 64.96 & 90.00 & 77.48 \\ \midrule
\rowcolor{blue!5}\multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{Ours} & \textbf{67.92} & 89.60 & \textbf{78.76} \\ \midrule
\multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{Ours} & 67.20 & \textbf{90.00} & 78.60 \\ \midrule
\multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{Ours} & 67.68 & 89.60 & 78.64\\ \bottomrule[1.5pt]
\end{tabular}
}
\label{tab_model_ablation}
\end{table}

